Enumeration of minimal acyclic automata via generalized parking functions

We give an exact enumerative formula for the minimal acyclic deterministic finite automata. This formula is obtained from a bijection between a family of generalized parking functions and the transitions functions of acyclic automata.

==> adfa.tex <==
%    %%
% \paragraph{}
% In the following, the start to recall the result of
% \cite[Theorem 3.1]{liskovets2006exact} about exact enumeration of ADFA. Then one
% defines a bijection $\bij$ between \emph{transition functions} $\delta$ of
% ADFAs over an alphabet of $k$ symbols and $m^k$-parking functions. The core of
% this bijection induces an interesting characterization of states right language
% and give us a natural way to compute the number of structures $(A, \delta)$ of
% ADFA \emph{simples} and \emph{coreachable}. From that we adapt the technique
% \cite[Theorem 3.2]{liskovets2006exact} (use to enumerate ``\emph{initially
% connected acyclic automata}''/structures $(i, \delta)$ of ADFA) to enumerate
% \emph{minimal} ADFA.
% \begin{table}
% \begin{center}
% \begin{tabular}{r|c|l|l||l}
%                        & Structures       & Notations   & Enumeration & Parking functions\\
%                        \hline 
%  ADFA                  & $(i,A, \delta)$  &             & $\adfa_k$ & $\PF^\bullet(2m^k)$\\ \hline
%  Transitions functions & $\delta$         & $\tADFA_k$  & $\tadfa_k$ & $\PF(m^k)$\\
%  \hline
%  Non-initial ADFA      & $(A, \delta)$    & $\tfADFA_k$ & $\tfadfa_k$ & $\PF(2m^k)$\\
%  Simple coreachable non-initial ADFA
%                        & $(A, \delta)$    & $\tfsADFA_k$& $\tfsadfa_k$ & $\SPF(2m^k-1)$\\
%  \hline
%  Extended ADFA         & $(A, \delta, T)$ & $\eADFA^T_k$  & $\eadfa_k^t$ & $\PF(2(m+t)^k-t-1)$\\
%  Simple extended ADFA  & $(A, \delta, T)$ & $\esADFA^T_k$& $\esadfa_k^{\,t}$ & $\SPF(2(m+t)^k-t-1)$\\
%  \hline  
%  Minimal ADFA          & $(i,A, \delta)$  &              & $\madfa_k$  
% \end{tabular}
% \end{center}
% \caption{Summary of notations and bijections of generalized parking
% functions (with $\PF^{\bullet}(\seqPF)$ the pointing (of species
% \cite{bergeron1998combinatorial}) in $\PF(\seqPF)$).}
% \end{table}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Enumeration of transition functions}
% \label{ssec:enumeration_of_transition_functions}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In \cite{liskovets2006exact}, V. \textsc{Liskovets} gives an enumeration of all 
% acyclic deterministic finite automata (ADFA) by enumerating those 
% \textit{transition functions}:
% \begin{align*}
%     \tadfa_k(n) &= \sum_{j=0}^{n-1}(-1)^{n-j-1}\binom{n}{j}(j+1)^{k(n-j)}
%                    \tadfa_k(j)\,.
%     \tag*{\cite[Theorem 3.1]{liskovets2006exact}}
% \end{align*}
% We denote $\tADFA_k[n]$ the underlying transitions 
% functions set of ADFA.
% \begin{remarq}
%     That formula gives a trivial ADFA enumeration formula: 
%     $\adfa_k(n) = n 2^n\tadfa_k(n)$.
% \end{remarq}
% \begin{thm}
%     There is a bijection between the structures $\PF(m^k)$ and $\tADFA_k$.
% \end{thm}
% \begin{preuve}
%     From (\ref{eq:sg_pf_k}), the increasing map $\seqPF$ defined by $\seqPFn{m}
%     = m^k$ gives us:
%     \begin{align*}
%         f_n &= \sum_{j=1}^n (-1)^{j-1}\binom{n}{j} (n-j+1)^{kj}f_{n-j} =
%             \tadfa_k(n)\,.
%     \end{align*}
% \end{preuve}
% Now, one gives an explicit bijection $\bij$ between both structures.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Linear order on parking functions}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Let $(Q_i)$ be a $\PF(2m^k)$-structure.
% One consideres the natural order on $[n]$: $1 <
% 2 < \cdots < n$ and build new one $<_q$ on $[n]$ from the sequence $(Q_i)$:
% \begin{align*}
%     i <_q j \quad\Longleftrightarrow\quad \begin{dcases*}
%         i \in Q_{k}\; \text{and}\; j \in Q_{k'} & with $k < k'$ or\\
%         i, j \in Q_k & and $i < j$\,.
%     \end{dcases*} 
% \end{align*}
% \begin{table}
% \begin{ex}
%     \label{ex:order_pf_structures}
%     The following $\PF(m^2)$-structures on $[4]$:
%     \begin{align*}
%         \boldsymbol{(}\,
%         4\mid 12\mid \cdot\mid \cdot\mid \cdot\mid \cdot\mid \cdot\mid \cdot\mid \cdot\mid 3\mid \cdot\mid \cdot\mid \cdot\mid \cdot\mid \cdot\mid \cdot
%         \,\boldsymbol{)}
%     \end{align*}
%     defines the order $4 <_q 1 <_q <_q 2 <_q 3$ and this one on $[5]$:
%     \begin{align*} 
%     \boldsymbol{(}\,
%     3\mid\cdot\mid\cdot\mid25\mid\cdot\mid\cdot\mid\cdot\mid\cdot\mid\cdot\mid\cdot\mid\cdot\mid\cdot\mid\cdot\mid\cdot\mid1\mid\cdot\mid\cdot\mid\cdot\mid\cdot\mid\cdot\mid4\mid\cdot\mid\cdot\mid\cdot\mid\cdot
%     \,\boldsymbol{)}
%     \end{align*}
%     defines the order $3 <_q 2 <_q 5 <_q 1 <_q 4$.
% \end{ex}
% \end{table}
% \begin{remarq}
%     The order $<_q$ is the linear order defined the inverse of the
%     standardization of the parking functions seen as a word. (In the previous
%     example the first parking function could be represented by the word
%     $22\substack{1\\0}1$ and the inverse of it standardization is $4123$, same
%     for the second $std(\substack{1\\5}41\substack{2\\1}4)^{-1} = 32514$.)
% \end{remarq}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Transition function from parking function}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Considering the \emph{cutting factor} $(F_j)_{j \in [n]}$ of $(Q_i)$ 
(\SOld \ref{ssec:cutting_factors})
defines by $F_j = (Q_i)_{i \in [(j-1)^k+1, j^k]}$:
\begin{align}
    \boldsymbol{(}\,
    \underbrace{Q_1}_{F_1} \boldsymbol{\mid} 
    \underbrace{Q_2 \mid \cdots \mid Q_{2^k}}_{F_2}  \boldsymbol{\mid} 
    \underbrace{Q_{2^k+1} \mid \cdots \mid Q_{3^k}}_{F_3} \boldsymbol{\mid} 
    \underbrace{Q_{3^k+1} \mid \cdots \mid Q_{4^k}}_{F_4} \boldsymbol{\mid} 
    \cdots \,\boldsymbol{)}
    \label{eq:split_factors}
\end{align}
By definition, $F_i$ is a sequence of $i^k - (i-1)^k$ sets and one remarks
this is exactly the number of distincts maps $\nu : U \to V$ with $\card{U} = k$ 
and $\card{V} = i$ and there exists $u \in U$ such that $\nu(u) = v$ for $v \in V$ 
fixed.

So we associate to each subsequence $F_i$ all the maps $\nu^{(i)}$ on $\Sigma$
into the set of state $\{\emptyset\} \cup \{q_1 \cdots q_{i-1}\}$ such that
there always exists at least one symbol $a$ such as $\nu^{(i)}(a) =
q_{i-1}$.
Furthermore, for a fixed order on $\Sigma$: $a_1 < a_2 < \cdots < a_k$, we define a
total order on the maps $\nu$ using the lexicographical order defined by $<_q$
on the words $\nu^{(i)}(a_1)\nu^{(i)}(a_2)\cdots \nu^{(i)}(a_k)$. This order on
maps $\nu^{(i)}_{1} < \cdots < \nu^{(i)}_{i^k - (i-1)^k}$ gives us a
deterministic way to associate to each set $Q_{(i-1)^k+j}$ of $F_i$ exactly one
map $\nu$, the map $\nu^{(i)}_j$:

\begin{minipage}[t]{.6\textwidth}
\begin{align*}
\begin{array}{c||lllll||l}
          & a_1       & a_2       & \cdots & a_{k-1}   & a_k       & \Sigma                    \\
\hline\hline
Q_1       & \emptyset & \emptyset & \cdots & \emptyset & \emptyset & \nu^{(1)}_1           \\
\hline
Q_2       & \emptyset & \emptyset & \cdots & \emptyset & q_1       & \nu^{(2)}_1           \\
Q_3       & \emptyset & \emptyset & \cdots & q_1       & \emptyset & \nu^{(2)}_2           \\
\vdots    &           &           & \vdots &           &           & \vdots                 \\
Q_{2^k}   & q_1       & q_1       & \cdots & q_1       & q_1       & \nu^{(2)}_{2^k-1}     \\
\hline
Q_{2^k+1} & \emptyset & \emptyset & \cdots & \emptyset & q_2       & \nu^{(3)}_1           \\
Q_{2^k+2} & \emptyset & \emptyset & \cdots & q_1       & q_2       & \nu^{(3)}_2           \\
\vdots    &           &           & \vdots &           &           & \vdots                \\
Q_{3^k}   & q_2       & q_2       & \cdots & q_2       & q_2       & \nu^{(3)}_{3^k - 2^k} \\
\hline
\vdots    &           &           & \vdots &           &           & \vdots                      
\end{array}
\end{align*}
From the association $Q_{(i-1)^k+j}$ with $\nu^{(i)}_{j}$, the map $\bij$ 
associates a map $\delta : [n] \times \Sigma \to [n] \cup \{\emptyset\}$ to each 
$\PF(m^k)$-structures $(Q_i)$ on $[n]$ defined by:  
\end{minipage}
\hfill
\noindent
\begin{minipage}[t]{.35\textwidth}
\begin{ex}
    From Example \ref{ex:order_pf_structures}, the $\PF(m^2)$-structure on $[4]$:
\begin{align*}
\begin{array}{c|c||ll||l}
\multicolumn{2}{c||}{} & a_1       & a_2       &   \Sigma                    \\
\hline\hline
Q_1   & 4      & \emptyset & \emptyset & \nu^{(1)}_1           \\
\hline
Q_2   & 12     & \emptyset &   4       & \nu^{(2)}_1           \\
Q_3   & \cdot  &   4       & \emptyset & \nu^{(2)}_2           \\
Q_4   & \cdot  &   4       &   4       & \nu^{(2)}_3 \\
\hline
Q_5   & \cdot  & \emptyset &   1       & \nu^{(3)}_1     \\
Q_6   & \cdot  &   4       &   1       & \nu^{(3)}_2           \\
Q_7   & \cdot  &   1       & \emptyset & \nu^{(3)}_3           \\
Q_8   & \cdot  &   1       &   4       & \nu^{(3)}_4           \\
Q_9   & \cdot  &   1       &   1       & \nu^{(3)}_5 \\
\hline
Q_{10}& 3      & \emptyset &   2       & \nu^{(4)}_1 \\
\vdots& \vdots & \vdots    & \vdots    & \vdots \\
Q_{16}& \cdot  &  2        &   2       & \nu^{(4)}_7                
\end{array}
\end{align*}
\end{ex}
\end{minipage}
\begin{align*}
    \delta(q, a) = \nu^{(i)}_{j}(a) \qquad\quad \text{with}\quad q \in Q_{(i-1)^k +
    j}\,.
\end{align*}
\begin{thm}
    \label{thm:bij_PF_ADFA}
    The map $\bij$ is a bijection between $\PF(m^k)$ and $\tADFA_k$. 
\end{thm}
\begin{preuve}
    The construction $\bij$ asserts if $\delta(q, a) = q'$ then $q' <_q q$ for 
    any $q \in [n]$ and any $a \in \Sigma$, so $\delta$ is in $\tADFA_k$. Reciprocally 
    to any $\delta$ of $\tADFA_k$, that is easy to define the order $<_q$ 
    by induction from states $q$ such that $\delta(q,a) = \emptyset$ for any 
    $a \in \Sigma$. This order defines a sequences $(Q_i)$ and that is satisfying 
    parking function condition (\ref{eq:pf_condition}).  
\end{preuve}
\begin{table}
\begin{ex}
    The second $\PF(m^2)$-structure on $[5]$ of Example 
    \ref{ex:order_pf_structures} is associated by $\bij$ to the transition 
    function (with $\Sigma = \{a, b\}$) represented by:
    \begin{center}
%%%%% e < 3 < 2 < 5 < 1 < 4
%%%%%%% a b
%3      e e  1
%%%%%%%%%%%%
%\cdot  e 3  2
%\cdot  3 e  3
%25     3 3  4
%%%%%%%%%%%%
%\cdot  e 2  5
%\cdot  3 2  6
%\cdot  2 e  7
%\cdot  2 3  8
%\cdot  2 2  9
%%%%%%%%%%%%
%\cdot  e 5  10
%\cdot  3 5  11
%\cdot  2 5  12
%\cdot  5 e  13
%\cdot  5 3  14
%1      5 2  15
%\cdot  5 5  16
%%%%%%%%%%%%
%\cdot  e 1  17
%\cdot  3 1  18
%\cdot  2 1  19
%\cdot  5 1  20
%4      1 e  21
%\cdot  1 3  22
%\cdot  1 2  23
%\cdot  1 5  24
%\cdot  1 1  25
{\newcommand{\AOnooo}{\node (0){$\emptyset$}
;}\newcommand{\AOnooa}{\node (1) [circle, draw] {$3$}
;}\newcommand{\AOnoob}{\node (2) [circle, draw] {$2$}
;}\newcommand{\AOnooc}{\node (3) [circle, draw] {$5$}
;}\newcommand{\AOnood}{\node (4) [circle, draw] {$1$}
;}\newcommand{\AOnooe}{\node (5) [circle, draw] {$4$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=1cm, row sep=.1cm]{
                &  & \AOnoob \\ 
 \AOnooe &        \AOnood        &  \AOnooc  & \AOnooa & \AOnooo \\  
};
\path[->] (3) edge node[swap] {$\scriptstyle a,b$} (1)
          (5) edge node {$\scriptstyle a$} (4)
          (4) edge node[swap] {$\scriptstyle a$} (3)
          (5) edge[bend right] node[swap] {$\scriptstyle b$} (0)
          (2) edge node {$\scriptstyle a,b$} (1)
          (4) edge node {$\scriptstyle b$} (2)
          (1) edge node {$\scriptstyle a,b$} (0);
\end{tikzpicture}}
    \end{center} 
\end{ex}
\end{table}
\begin{remarq}
    \label{rq:bij_k_1_rooted_trees}
    For $k=1$, the map $\bij$ defined one of the bijections between
    (usual) parking functions and rooted trees.
\end{remarq}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Non-initial ADFA} \label{ssec:Non_initial_ADFA}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The main interest of this construction is each set $Q_j$ of the parking 
function $(Q_i)$ encodes exactly the transitions of states $q \in Q_j$. This is 
almost the notion of right language, and to encode exactly this notion, we need 
to distinguish which states are \textit{accepting} and which are not. So in this 
section we considere the \emph{non-initial ADFA} over an alphabet of $k$ symbols,
noted $\tfADFA_k$.   

The idea is to split a parking function each set in two: one for 
\textit{accepting states} and one for the others, both associated to the same 
transitions:
\newcommand{\qqq}[1]{\vcenter{\hbox{\tikz[remember picture] \node (q#1){$Q_{#1}$};}}}
\newcommand{\qqr}[1]{
    \substack{\vcenter{\hbox{\tikz[remember picture] \node (rf#1){$R_{#1}$};}}\\
    \vcenter{\hbox{\tikz[remember picture] \node (r#1){$R_{#1}'$};}}}
}
\begin{align*}
\begin{aligned}
    &\vcenter{\hbox{\tikz[remember picture] \node (lp) {$\boldsymbol{(}$};}}\,
        \qqq{1} \boldsymbol{\mid}
        \qqq{2} \boldsymbol{\mid} 
        \qqq{2^k+1} 
        \mid \cdots \mid 
        \qqq{3^k} \boldsymbol{\mid} 
        \qqq{3^k+1} 
        \mid \cdots \mid 
        \qqq{4^k} \boldsymbol{\mid} 
    \cdots \,\boldsymbol{)}\\
    &\vcenter{\hbox{\tikz[remember picture] \node (lp2) {$\Bigg($};}}\,
        \qqr{1} \boldsymbol{\mid}
        \qqr{2} \boldsymbol{\mid} 
        \qqr{2^k+1} 
        \mid \cdots \mid 
        \qqr{3^k} \boldsymbol{\mid} 
        \qqr{3^k+1} 
        \mid \cdots \mid 
        \qqr{4^k} \boldsymbol{\mid} 
    \cdots \,
    \Bigg) \substack{\tikz \node {$\subset A\hphantom{;;;;}$};\\ 
                     \tikz \node {$\subset [n]\backslash A$};}
\end{aligned}
    %\label{eq:schema_splitting}
\end{align*}
\newcommand{\qqs}[1]{
    \path[overlay,->] (q#1.west) edge[bend right=10] (rf#1.west)
                                edge[bend right=10] (r#1.west);
}
\begin{tikzpicture}[remember picture]
    \path[overlay,->, thick] (lp.west) edge[bend right] (lp2.west);
    \qqs{1}\qqs{2}\qqs{2^k+1}\qqs{3^k}\qqs{3^k+1}\qqs{4^k}
\end{tikzpicture}
In terms of $\seqPF$-parking functions double which state is equivalent to
considere the increasing map defined by $m \mapsto 2\seqPF(m)$:
\begin{prop}
    \label{prop:2mk_pf_F_delta}
    The structures $\PF(2m^k)$ and $\tfADFA_k$ are isomorphics.
\end{prop}
\begin{preuve}
    Thanks to \cite[Corollary 5.6]{kung2003goncarov}\todo{+papier}, one has
    $\card{\PF_n(2m^k)} = 2^n\card{\PF_n(m^k)}$ so one has $\PF(2m^k)$
    is isormophics to non-initial ADFA.
\end{preuve}
This isomorphism is immediate from the definition of $\seqPF$-parking functions
in terms of recursive grammar (\ref{eq:pf_definition_constructive}).
Furthermore, we give a generalization $\bij_A$ of $\bij$ defined by: the factors
$F_j = (Q_i)$ with $i$ between $2(j-1)^k +1$ and $2j^k$ (as the \emph{cutting 
factors} of $(Q_i)$), we associate to $Q_{2(i-1)^k+2j}$ and $Q_{2(i-1)^k+2j+1}$ 
the map $\nu_j^{(i)}$, finally one defines the structures $(A, \delta)$ with 
$\delta$ defined in the same way, and $A = \bigcup_{i \in [n^k]} Q_{2i-1}$ is 
the union of all odd sets.

Now the \emph{cutting factor} of $(Q_i)$ involves an information similar to the
height property use to define an efficient minimization algorithm in
\cite{revuz1992minimisation}:
\begin{lemme}
    \label{lem:non_initial_ADFA_simple}
    A non-initial ADFA is \emph{simple} if and only if $\card{Q_i} \ieq 1$, for
    any $i$.
\end{lemme}
\begin{preuve}
    The \textit{cutting factor} defines height notion related to the
    \emph{absorbing state} and by induction on $F_j$, one deduces that if there
    exists $q$ and $r$ (in $Q_j$ and $Q_k$) are right language equivalents if
    and only if there exists $q'$ and $r'$ in $Q_i$ with $i \ieq \min(j,k)$.
\end{preuve}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Coreachage non-initial automata}
\label{ssec:coreachable_non_init_automata}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $(A, \delta)$ be a non-initial ADFA and let $(Q_i)$ be the $2m^k$-parking
function such that $\bij_A(Q_i) = (A, \delta)$.
  
Moreover this traduction in terms of parking functions spotlights the sets
$(Q_1, Q_2)$ of the first factor $F_1$ of the \textit{cutting factor}
represents states $q$ such that $\delta(q, \Sigma) = \{\emptyset\}$ (with $Q_1
\subset A$ and $Q_2 \subset [n] \backslash A$), and with a similar proof of the
Lemma \ref{lem:non_initial_ADFA_simple} we show:
\begin{lemme}
    The non-initial ADFA $(A, \delta)$ is \emph{coreachable} \emph{if and only
    if} the $2m^k$-parking functions satisfy $Q_2 = \emptyset$.
\end{lemme}
In others terms this Lemma involves to considere $2m^k$-parking functions with
one contraint on the first part of the cutting factor. Obviously that is
equivalent to considere generalized parking functions $(Q_i)$ on $[n]$ which are
sequence of $(2n^k-1)$-sets. The bijection between $\PF(2m^k)$-structures and
those others and the grammar \ref{eq:pf_definition_constructive} lead us to
define $\seqPF$: the fact to append an emptyset in the first cutting factor
$F_1$ involves $\seqPF(m) := 2m^2-1$.
\begin{coro}
    \label{cor:coreachable_non_initial_ADFA_2mk_1_PF}
    \emph{Coreachable non-initial ADFA} are isomorphics to $(2m^k-1)$-parking
    functions.
\end{coro}
We denote $\tfADFA_k$ the \emph{coreachable non-initial ADFA} over an alphabet
of $k$ symbols. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Simple coreachage non-initial automata}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The bijection $\bij_A$ involves an interesting characteristic of the right
language of ADFA states translates on sets $Q_i$ of the associated
$2m^k$-parking functions. As corollary of Lemma
\ref{lem:non_initial_ADFA_simple} one deduces:
\begin{coro}
    \label{cor:non_initial_ADFA_simple}
    A non-initial ADFA $(A, \delta)$ is \emph{simple} \textit{if and only if}
    $\bij_A^{-1}(A, \delta)$ is a \emph{simple} $2m^k$-parking functions.
\end{coro}
From Corollaries \ref{cor:coreachable_non_initial_ADFA_2mk_1_PF}
and \ref{cor:non_initial_ADFA_simple}, one obtains:
\begin{lemme}
    \label{lem:coreachable_simple_non_initial_ADFA_2mk_1_SPF}
    The \emph{non-initial ADFA simple} and \emph{coreachable} are isomorphics to
    \emph{simple $(2m^k-1)$-parking functions}.
\end{lemme}
We denote $\tfsADFA_k$ the non-initial ADFA simple and coreachable over an
alphabet of $k$ symbols.
As a consequence, the (non-labelled) enumeration of $\tfsADFA_k$ is given by
the enumeration of simple parking functions (\ref{eq:sg_simple_pf}):
\begin{align*}
    \tfsadfa_k(n) = \sum_{\substack{\tau \models n\\ \tau_1 = 1}}
    \prod_{i = 2}^{\ell(\tau)} \binom{2 \left[ (1+\tau(i-1))^k -
    (1+\tau(i-2))^k\right]}{\tau_i}
\end{align*}
where $\tau(i)$ is the partial sum $\tau_1 + \cdots + \tau_i$ of parts of
$\tau$ (with $\tau(0) = 0$).

There is the firsts coefficients of $\tfsadfa_k$ (as ordinary generating
series (\cf Remark \ref{rq:simple_parking_functions_trivial_automorphism})) for
$k = 1$, $2$ and $3$.
\begin{center}
$\begin{array}{c|l|l|l|l|l|l|l|l||c}
k \backslash n & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & \textit{OEIS} \\ 
\hline
1 & 1 & 1 & 2  & 5    & 14      & 42          & 132        & 429  & \oeis*{A000108}\\
2 & 1 & 1 & 6  & 75   & 1490    & 41415       & 1495806    & 66908663\\
3 & 1 & 1 & 14 & 623  & 59766   & 10182221    & 2740931060 & 1078233863119
\end{array}$
\end{center}
\begin{remarq}
    The bijection $\bij_A'$ apply to simple $(2m-1)$-parking functions produces
    binary trees rooted by the \textit{unique (accepting)} state $q$ such that
    $\delta(q, a) = \emptyset$ (the order left and right child is fixed by the
    status of \textit{accepting state}). (There is a species bijection between
    $\SPF(2m-1)$-species and binary trees species.) 
\end{remarq}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Extended ADFA}
%%%%%%%%%%%%%%%%%%%%%%%%%%
The idea of this section is to define a bijection between simple
coreachable non-initial ADFA and couple of structures $(e, m)$ with $e$ an
``extended ADFA'' (with a well choosen definition) and $m$ a minimal ADFA,
similary to the idea uses in \cite[Theorem 3.2]{liskovets2006exact} to enumerate
structures $(i,\delta)$ (``initially connected acyclic automata'').
Let $\aut = (A, \delta)$ be a simple coreachable non-initial ADFA.  
One consideres a substructure $\aut^{(i)} = (i, A', \delta')$ of $\aut$ defined
by: $A'$ and $\delta'$ are the restriction (of $A$ and $\delta$) to all
reachable states from $i$. That implies
\begin{prop}
    The substructure $\aut^{(i)}$ is \emph{minimal} ADFA.
\end{prop}
\begin{preuve}
    By definition $\aut$ is a simple coreachable non-initial ADFA, so by
    construction $\aut^{(i)}$ is reachable, coreachable and simple. 
\end{preuve}
Now for a well choosen construction, our goal is to describe
$\tfsADFA_k$-structures as couple of minimal ADFA $\mADFA_k$ and extended ADFA
$\esADFA_k$.%, like in \cite{liskovets2006exact}.
% \begin{align*}
%     \tfsADFA_k [n] := \sum_{\substack{S \sqcup T = [n]\\  t :=\card{T} > 0}} 
%                       \esADFA^{t}_k [S] \cdot \mADFA_k [T]\,
% \end{align*}
% fixed a initial state $i$, for $n \seq 1$.
We define \emph{extended ADFA} in the same way of the ``quasi acyclic automata''
in \cite[\SOld 2.15]{liskovets2006exact} adding some constraints $C$ in the
same way of section \ref{ssec:coreachable_non_init_automata}.
Let $C = (\nu_i,F_i)_{i \in [t+1]}$ a family of constraints (defined below).
An \emph{extended ADFA} $\eADFA_k^C$ on $n$ states over an alphabet $\Sigma$
compelled to the constraints $C$ is a tuple $(A, \delta)$ with $\delta$ is an
extended transition function:
\begin{align*}
    \delta : [n] \times \Sigma &\to [n] \cup \{\emptyset\} \cup \{\alpha_i \mid
    i \in [t]\}
%\end{align*}
\intertext{
with $\alpha_i$ are \emph{extra absorbing states} and the family $(\nu_i,F_i)$
are maps marked accepting or not:}
%\begin{align*}
    \nu_i : \Sigma &\to \{\emptyset\} \cup \{\alpha_i \mid i \in [t]\}\quad
    \text{and}\quad F_i \; \text{is \textit{true} or \textit{false}}
\end{align*}
defining constraints on $\delta$ which are: for any constraint $(\nu_i,F_i)$,
there exists $a \in \Sigma$ such that $\delta(q, a) \neq \nu(a)$, for any 
$q \in A$ if $F_i$ or any $q \in [n]\backslash A$ if not $F_i$.
Like with the DFA definition, we extend $\delta$ to words (with
$\delta^*(\alpha_i, a) = \alpha_i$) and we said $(A, \delta) \in \eADFA_k^C$ is
simple if there is no couple of distincts states $q$ and $r$ such that for any
word $w$, one has
\begin{align*}
    \delta(q, w) \in A \quad \textit{if and only if}&\quad \delta(r, w) \in
    A\,,\quad\text{and}\\
     \delta(q, w) = \delta(r, w) \in\, &\{\emptyset\}\cup \{\alpha_i \mid i \in
     [t]\}\,.
\end{align*}
This extended definition of ADFA could be express in terms of generalized
parking functions. If we forgive the notion of constraint, the fact to append
$t$ other \emph{absorbing states} is equivalent to considere a (simple)
$(2(m+t)^k)$-parking function, and that is easy to define a analogous bijection
to $\bij$ and $\bij_A$ (see sections
\ref{ssec:enumeration_of_transition_functions} and \ref{ssec:Non_initial_ADFA}).
Furthermore, like in section \ref{ssec:coreachable_non_init_automata}
considering $t+1$ constraints on absorbing states is equivalent to remove $t+1$
sets in the first factor of $(Q_i)$ cutting factors. So with analogy to
Corollary \ref{cor:non_initial_ADFA_simple} and Lemma
\ref{lem:coreachable_simple_non_initial_ADFA_2mk_1_SPF}:
%
\begin{lemme}
  (Simple) \emph{extended ADFA} $\eADFA_k^C$ ($\esADFA_k^C$) are bijections with
  (simple) $(2(m + t)^k - t - 1)$-parking functions. 
\end{lemme}
We denote $\eadfa_k^t$ and $\esadfa_k^{\ t}$ the enumeration formula of
respectively the extended ADFA $\eADFA_k^C$ and $\eADFA_k^C$ with $C$ a set of $t+1$
constraints. Let $\aut$ be a simple coreachable non-initial ADFA and let
$\aut^{(i)}$ be the minimal defined from $i$ such that $i$ reachs the $t$
states $U$ in $\aut$. One defines the complementary $\widebar{\aut}^{(i)} =
(A', \delta')$ of $\aut^{(i)}$ as the simple extended ADFA compelled to the
constraints $(\nu_i, F_i)_{i \in [t+1]}$:
\begin{align*}
    \nu_{can(q)}&\quad \text{defined by}\quad \nu_{can(q)}(a) := \delta(q,
    a)\quad \text{with}\; a \in \Sigma\,,\qquad \text{and}\qquad
    F_i := q \in A\,,
\end{align*}
for any state $q$ in $\aut^{(i)}$ with $can(q)$ the image of $q$ from the unique
order-preserving bijection between two sets of integers: $[t]$ and $U \subset
[n]$ of $t$ states. We add an extra constraint to be coherent with coreachable
ADFA: $\nu_{t+1}(a) = \emptyset$ for any $a$ and $F_{t+1}$ false. Then one
defines $A' := A \cap U$ with $U$ and $\delta'$:
\begin{align*}
    \delta'(q, a) := \begin{dcases*}
        \delta(q, a) & if $\delta(q, a) \notin U$,\\
        \alpha_{can(\delta(q,a))} & in otherwise.
    \end{dcases*}
\end{align*}
This construction induces a bijective transformation between $\aut$ and
$(\aut^{(i)}, \widebar{\aut}^{(i)})$ for $i$ fixed (see Example
\ref{ex:decomposition_of_simple_coreachable_non_initial_ADFA}). We denote
$\mADFA_k^C$ the set of minimal ADFA coherent with constraints $C$. A minimal
ADFA $\aut$ on set $U$ is coherent with $C$ ($\card{U} = \card{C}+1$) if for
each constraint $(\nu_i, F_i)$, the state $q = can^{-1}(i)$ has transitions and
accepting status:
\begin{align*}
    \delta(q, a) = \nu_i(a) \qquad\text{and}\qquad 
    q \in A \;\textit{iff}\; F_i\,.
\end{align*}
except the constraint $\delta(q, a) = \emptyset$ (for any $a$) and $q$ is not
accepting. This bijective transformation involves the combinatorial definition:
%
\begin{thm}
    Let $N$ be a set of states and let $i \in N$, one has:
    \begin{align*}
    \tfsADFA_k[N] &= \sum_{\substack{S\sqcup T = N\\ \card{T} = t \seq 1}}
                      \sum_{C \blacktriangleright S} 
                        \eADFA_k^C[S] \cdot \mADFA_k^C[T]
    \end{align*}
    with $C \blacktriangleright t$ the set of $t+1$ constraints $C$ (including
    those such that $\nu(a) = \emptyset$ for any $a$ and any absorbing status).
\end{thm}
So the set of minimal ADFA $\mADFA_k$ of $n$ states is given by $\mADFA_k[n] =
\sum_{C \blacktriangleright n} \mADFA_k^C[n]$. From the enumeration formula of
simple parking function (\ref{eq:sg_simple_pf}) one has the enumeration formula
(similar to \cite[Theorem 3.2]{liskovets2006exact}):
\begin{coro}
    For $i$ a fixed state,
    \begin{align*}
    \tfsadfa_k(n) = \sum_{t=1}^n 
        \binom{n-1}{t-1}\esadfa_k^{\ t}(t)\madfa_k(n-t)\,. 
    \end{align*}
\end{coro}
There is the first coefficients of $\madfa_k$ for $k=1$, $2$, $3$ and $4$:
\begin{center}
$\begin{array}{c|l|l|l|l|l|l|l||c}
k \backslash n & 1 & 2 & 3 & 4 & 5 & 6 & 7  & \textit{OEIS} \\ 
\hline
1 & 1 & 2  & 4    & 8       & 16         & 32            & 64                \\
2 & 1 & 6  & 60   & 900     & 18480      & 487560        & 15824880         \\
3 & 1 & 14 & 532  & 42644   & 6011320    & 1330452032    & 428484011200     \\
4 & 1 & 30 & 3900 & 1460700 & 1220162880 & 1943245777800 & 5307146859111120 
\end{array}$
\end{center}
\begin{figure}
\begin{ex}\label{ex:decomposition_of_simple_coreachable_non_initial_ADFA} 
Let $\aut \in \tfsADFA_2[9]$ be an simple coreachable non-initial
ADFA on the left and the decomposition $(\aut^{(5)}, \widebar{\aut}^{(5)})$ for
the fixed state $5$. The minimal ADFA $\aut^{(5)}$ is represented at the top
and its complementary at the bottom, both at the right. The complementary is an
element of $\eADFA_k^C$ with $C$ defined from transitions and states of
$\aut^{(i)}$: there is no state $q$ such that $\delta(q,a) = \emptyset$ and
$\delta(q,b) = \alpha_{can(1)} = \alpha_1$ with $q \in A$ (description of
state $2$); or $\delta(q, a) = \alpha_{can(4)} = \alpha_{3}$ and $\delta(q, b) =
\alpha_{can(2)} = \alpha_2$ with $q \notin A$ (description of state $9$);
\textit{etc}; or $q \notin A$ and $\delta(q,a) = \delta(q,b) = \emptyset$ (the
forced constraint).

\begin{minipage}[t]{.45\textwidth}\vspace{0pt}
\begin{center}
\scalebox{.8}{\newcommand{\AOnooo}{\node (0) [circle, draw, double] {$1$}
;}\newcommand{\AOnooa}{\node (1) [circle, draw, double] {$3$}
;}\newcommand{\AOnoob}{\node (2) [circle, draw, double] {$2$}
;}\newcommand{\AOnooc}{\node (3) [circle, draw, double] {$4$}
;}\newcommand{\AOnood}{\node (4) [circle, draw] {$5$}
;}\newcommand{\AOnooe}{\node (5) [circle, draw] {$7$}
;}\newcommand{\AOnoof}{\node (6) [circle, draw] {$8$}
;}\newcommand{\AOnoog}{\node (7) [circle, draw] {$9$}
;}\newcommand{\AOnooh}{\node (8) {$\emptyset$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=1cm, row sep=.5cm, ampersand replacement=\&]{
 \AOnoob  \&\AOnooe \& \AOnooo \&  \AOnooh \\ 
  \AOnoog \&        \& \AOnooc \&  \\ 
 \AOnood  \&\AOnooa \&         \& \AOnoof \\ 
};
\path[->] 
     (2) edge[bend left=40] node[swap] {$\scriptstyle b$} (0)
	 (6) edge node[swap] {$\scriptstyle a$} (8)
	 (2) edge[bend left=40] node {$\scriptstyle a$} (8)
	 (7) edge node {$\scriptstyle a$} (3)
	 (4) edge node[swap] {$\scriptstyle b$} (7)
	 (7) edge node[swap] {$\scriptstyle b$} (2)
	 (6) edge node {$\scriptstyle b$} (3)
	 (0) edge node {$\scriptstyle b$} (8)
	 (1) edge node {$\scriptstyle a$} (6)
	 (4) edge[bend right=40] node {$\scriptstyle a$} (6)
	 (5) edge node {$\scriptstyle a$} (7)
	 (1) edge node[swap] {$\scriptstyle b$} (7)
	 (0) edge node[swap] {$\scriptstyle a$} (3)
	 (5) edge node {$\scriptstyle b$} (0)
	 (3) edge node[swap] {$\scriptstyle a,b$} (8);
\end{tikzpicture}}
\end{center}
\end{minipage}
\hfill\vrule\hfill
%\noindent
\begin{minipage}[t]{.5\textwidth}\vspace{0pt}
\begin{center}
\scalebox{.8}{\newcommand{\AOnooo}{\node (0) [circle, draw, initial] {$5$}
;}\newcommand{\AOnooa}{\node (1) [circle, draw] {$9$}
;}\newcommand{\AOnoob}{\node (2) [circle, draw] {$8$}
;}\newcommand{\AOnooc}{\node (3) [circle, draw, double] {$4$}
;}\newcommand{\AOnood}{\node (4) [circle, draw, double] {$2$}
;}\newcommand{\AOnooe}{\node (5) [circle, draw, double] {$1$}
;}\newcommand{\AOnoof}{\node (6) {$\emptyset$}
;}\begin{tikzpicture}[auto, initial text=]
\matrix[column sep=1cm, row sep=.5cm,ampersand replacement=\&]{
 \AOnooo \& \AOnooa \& \AOnood \& \AOnooe \\ 
         \& \AOnoob \& \AOnooc \& \AOnoof \\ 
};
\path[->] %(4) edge node {$\scriptstyle a$} (6)
	 (5) edge node[swap] {$\scriptstyle a$} (3)
	 (1) edge node {$\scriptstyle b$} (4)
	 (4) edge node {$\scriptstyle b$} (5)
	 (1) edge node {$\scriptstyle a$} (3)
	 (2) edge[bend right=40] node {$\scriptstyle a$} (6)
	 (2) edge node {$\scriptstyle b$} (3)
	 (3) edge node {$\scriptstyle a,b$} (6)
	 (0) edge node {$\scriptstyle b$} (1)
	 (5) edge node {$\scriptstyle b$} (6)
	 (0) edge node {$\scriptstyle a$} (2);
\draw[->] (4) .. controls (3.5,1.5) and (4,1.5) .. node {$\scriptstyle a$}(6);
\end{tikzpicture}} \\ \vfill \hrule \vfill
\scalebox{.8}{\newcommand{\AOnooo}{\node (0) [circle, draw, double] {$3$}
;}\newcommand{\AOnooa}{\node (1) [circle, draw] {$7$}
;}\newcommand{\AOnoob}{\node (2) {$\alpha_4$}
;}\newcommand{\AOnooc}{\node (3) {$\alpha_2$}
;}\newcommand{\AOnood}{\node (4) {$\alpha_1$}
;}\newcommand{\AOnooe}{\node (5) {$\alpha_3$}
;}\newcommand{\AOnoof}{\node (6) {$\alpha_5$}
;}\newcommand{\AOnoog}{\node (7) {$\alpha_6$}
;}\newcommand{\AOnooh}{\node (8) {$\alpha_7$}
;}\newcommand{\AOnooi}{\node (9) {$\emptyset$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=1cm, row sep=.5cm, ampersand replacement=\&]{
 \AOnoob \& \AOnooc \& \AOnooe \& \AOnoof \& \AOnooi \\ 
 \AOnood \& \AOnooa \& \AOnooh \& \AOnooo \& \AOnoog \\ 
};
\path[->] (0) edge node {$\scriptstyle a$} (7)
          (1) edge node {$\scriptstyle b$} (4)
          (0) edge node {$\scriptstyle b$} (8)
          (1) edge node {$\scriptstyle a$} (8);
\end{tikzpicture}}
\end{center}
\end{minipage}
\end{ex}
\end{figure}

==> parking_functions.tex <==
\bigskip
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Cycle index series and interpretation}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Non-commutative characteristic}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Like in \cite[§4 Equation 31]{novelli2008noncommutative}, one considere the
% non-commutative characteristic (in the complete $(\S^\pi$-basis of
% non-commutative symmetric functions) of $\seqPF$-parking functions on $[n]$,
% noted $F(\seqPF; n)$ as defined in \todo{citer papier}:
% \begin{align}
%     F(\seqPF; n) &= \sum_{\pi \models n} \alpha_\pi
%     \S^\pi 
%     \qquad\text{with}\quad
%     \alpha_\pi =\sum_{\tau \models \ell(\pi)}
%                     \prod_{i=1}^{\ell(\tau)} \binom{\pi(\seqPF; \tau,
%                     i)}{\tau_i}
%     \label{eq:characteristic_PF_n}
% \intertext{where $\pi \models n$ means $\pi$ is a composition of $n$, $\tau_i$
% means the $i^\text{th}$ part of $\tau$ and}
% %\begin{align*}
%     \pi(\seqPF; \tau, i) &:= 
%         \begin{dcases*}
%         \seqPFn{1 + \sum_{j = 1}^{\tau_1 + \cdots + \tau_{i-1}} \pi_j} -
%         \seqPFn{1 + \sum_{j = 1}^{\tau_1 + \cdots + \tau_{i-2}} \pi_j} & if $i
%         > 1$,\\
%         \seqPFn{1} & in otherwise.
%         \end{dcases*}\nonumber
% \end{align}
% This characteristic results of unrecursive translation of the cycle index series
% immediately induces by the recursive grammar
% (\ref{eq:pf_definition_constructive}).
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Interpretation}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We say a composition $I$ is the \emph{associated composition} of the
% $\seqPF$-parking function $(Q_i)$ if the sequence of cardinals $(q_j)$ of the
% subsequence $(Q_j)$ of non-empty sets of $(Q_i)$ is the composition $I$.
% \begin{prop}
%     \label{prop:characteristique_interpretation}
%     Each terms $\alpha_\pi S^\pi$ encodes all $\seqPF$-parking functions with
%     \textit{associated composition} is $\pi$.
% \end{prop}
% \begin{preuve}
%     The non-commutative characteristic of the species $\speciesSet$ restrict
%     to degree $n$ is $\S_n$. Now from the product of $S^\pi$ and the grammar
%     (\ref{eq:pf_definition_constructive}) that is immediate.
% \end{preuve}
% This interpretation gives us an easy way to enumerate specific parking
% functions, specially \emph{simple $\seqPF$-parking functions}.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Exponential generating series}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The change of basis in elementary basis $(\Lambda_\pi)$ of $F(\seqPF; n)$
% (\ref{eq:characteristic_PF_n}) gives us a formula \todo{citer papier + thm}
% which generalize the enumeration formula \cite[Theorem 4.2]{kung2003goncarov}:
% \begin{align}
%     \pf_\seqPF(t) = \sum_{n \seq 0} f_n\frac{t^n}{n!}\qquad\quad\text{with}
%     \quad f_n = \sum_{j=1}^{n}(-1)^{j-1}\binom{n}{j}\seqPFn{n-j+1}^{j}
%     f_{n-j}\,.
%     \label{eq:sg_pf_k}
% \end{align}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Simple parking functions}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A \emph{simple $\seqPF$-parking function} $(Q_i)$ is a $\seqPF$-parking
% functions such that $\card{Q_i} \ieq 1$ for any $i$. We denote $\SPF(\seqPF)$
% the species/set of simple $\seqPF$-parking functions.
% \begin{remarq}
%     \label{eq:pf_simple_id_permutations}
%     The simple $\seqPF$-parking functions for $\seqPF(n) = n$ are permutations. 
% \end{remarq}
% From the characteristic (\ref{eq:characteristic_PF_n}) and the interpretation
% (Proposition \ref{prop:characteristique_interpretation}) we deduce
% characteristic of $\SPF(\seqPF)$ on $[n]$, noted $S(\seqPF; n)$:
% \begin{align*}
%     S(\seqPF; n) &= \sum_{\tau \models \ell(\pi)}
%                     \prod_{i=1}^{\ell(\tau)} \binom{\tau(\seqPF; i)}{\tau_i} 
%                     \S^{1^n}
% \intertext{with}
%     \tau(\seqPF; i) &= \begin{dcases*}
%         \seqPFn{1 + \tau_1 + \cdots + \tau_{i-1}}
%     - \seqPFn{1 + \tau_1 + \cdots + \tau_{i-2}} & if $i > 1$,\\
%     \seqPFn{1} & in otherwise.
%     \end{dcases*}
% \end{align*}
% From this characteristic one obtains the enumeration formula of
% $\SPF(\seqPF)$-structures, the (exponential) generating series:
% \begin{align}
%     \spf_\seqPF(t) &= \sum_{n \seq 0} s_n t^n \qquad \text{with}\quad
%     s_n = \sum_{\tau \models n}
%     \prod_{i = 1}^{\ell(\tau)} \binom{\tau(\seqPF; i)}{\tau_i}\,.
%     \label{eq:sg_simple_pf} 
% \end{align}
% \begin{remarq}
%     \label{rq:simple_parking_functions_trivial_automorphism}
%     Contrary to $\PF(\seqPF)$ the species $\SPF(\seqPF)$ doesn't have
%     non-trivial automorphisms. So the generating series of structures and types
%     of isomorphisms of $\SPF(\seqPF)$ could be identified.
% \end{remarq}
% \begin{ex}
%     In $\PF_2(m^2)$ all parking functions are simples except
%     $\boldsymbol{(}12\mid \cdot\mid\cdot\mid\cdot\boldsymbol{)}$.
% \end{ex}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Cutting factors} \label{ssec:cutting_factors}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We define the \emph{cutting factors} of a $\seqPF$-parking function $(Q_i)$ on a
% set $[n]$ as the sequence of factor $(F_j)_{j \in [n]}$ with $F_j = (Q_i)$ with
% $i \in [\seqPFn{j-1}+1, \seqPFn{j}]$.
% \begin{ex}
%     The $\PF(m^2)$-structures $\boldsymbol{(}\; 3 \mid \cdot \mid 1
%     \mid \cdot \mid 2 \mid \cdot \mid \cdot \mid \cdot\mid \cdot
%     \;\boldsymbol{)}$ has the \textit{cutting factor} $(F_1,F_2,F_3)$ with $F_1
%     = (\,1\,)$, $F_2 = (\,\cdot \mid 1 \mid \cdot\,)$ and $F_3 =(\,2 \mid \cdot
%     \mid \cdot\mid \cdot \mid \cdot\,)$.
% \end{ex}

==> pf.tex <==
Parking functions were introduced in \cite{konheim1966occupancy} to modelize
hashing problem in computer sciences and appear in differents
context in combinatorics: \textit{labelled trees}, \textit{prüfer sequence}
\cite{moon1970counting}, \textit{hyperplane arrangements}
\cite{stanley1998hyperplane}, \textit{etc}. A parking function of degree $n$ is
a function $f : \NN_+ \to \NN_+$ such that $\card{f^{-1}([k])} \seq k$, for any
$k \in [n]$.

A generalization of parking function were formulated in
\cite{stanley2002polytope} and well studied in \cite{kung2003goncarov} \todo{+
nous}: let $\seqPF : \NN_+ \to \NN$ be an increasing map; a $\seqPF$-parking
function $f$ is a function $f$ such that $\card{f^{-1}([\seqPF(k)])} \seq k$.

\begin{remarq}
    The usual parking function are $\seqPF$-parking function with $\seqPFn{k} =
    k$.
\end{remarq}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Constructive definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
It is equivalent to consider a $\seqPF$-parking function $f$ of degree $n$ or a
sequence of $\seqPFn{n}$ sets $(Q_i)$ satisfying:
\begin{align*}
    \sum_{i = 1}^{\seqPFn{k}} \card{Q_i} \seq k\,,\quad\qquad \text{for any}\; k
    \in [n]\,.
\end{align*}
Both definition are simply in bijection by $f^{-1}(\{i\}) = Q_i$. In 
\todo{citer l'autre papier}, one defines $\seqPF$-parking functions, noted 
$\PF(\seqPF)$, as a constructive species \cite{bergeron1998combinatorial}
(that means a constructive class of labelled structures
\cite{flajolet2009analytic} endowed of an action of symmetric group):
\begin{align}
    \PF(\seqPF) = (\speciesSet^{\seqPFn{1}})_0 + \sum_{n \seq 1}
    (\speciesSet^{\seqPFn{1}})_n \cdot \PF(\rho_n)\qquad \text{with}\;
    \rho_n(k) = \seqPFn{n + k} - \seqPFn{1}\,;
    \label{eq:pf_defition_constructive}
\end{align}
with $\speciesSet$ the species of sets ($\speciesSet[U] = \{U\}$ for any finite
set $U$); $\cdot$ the product/concatenation of species ($(\speciesA \cdot
\speciesB)[U] = \sum_{S \sqcup T = U} \speciesA[S] \times \speciesB[T]$, for
any species $\speciesA$ and $\speciesB$, and any finite set $U$); and
$(\speciesSet^{\seqPFn{1}})_n$ means the species obtains by restriction of
$\speciesSet^{\seqPFn{1}} = \speciesSet \cdots \speciesSet$ to sets of
cardinality $n$. We denote $\PF_n(\seqPF) := \PF(\seqPF)[n]$ the
$\PF(\seqPF)$-structures on the set $[n] = \{1, \cdots, n\}$.

In the following, we will be focus on $\seqPF$ defined by $\seqPFn{n} = n^k$
with $k \in \NN$ and some analogous families with $\seqPFn{n} = (n+r)^k - 1$
(with $r \seq 1$).

The first family of parking functions ($\seqPFn{n} = n^k$) is in bijection
the transitions functions of deterministic acyclic finite automata on alphabets
of $k$ letters (and only $1$ \textit{sink}) \todo{ref sec/thm}.
Let us denote $\PF^k$ the $\seqPF$-parking functions for $\seqPFn{n} = n^k$.
\begin{ex}
    The first structures $\PF^2_n$ for $n=1, 2$ and $3$:
\begin{align*}
    \PF^2_1 &= \left\{
        1
    \right\}\,,\qquad
    \PF^2_2 = \left\{
    12,\; 21,\; 13,\; 31,\; 14,\; 41,\; 11
    \right\}\,,\\
    \PF^2_3 &= \left\{\begin{array}{l}
123,\; 312,\; 132,\; 213,\; 321,\; 231,\; 124,\; 412,\; 142,\; 214,\; 421,\; 241,\; 134,\; 413,\; 143,\; \\
314,\; 431,\; 341,\; 125,\; 512,\; 152,\; 215,\; 521,\; 251,\; 135,\; 513,\; 153,\; 315,\; 531,\; 351,\; \\
145,\; 514,\; 154,\; 415,\; 541,\; 451,\; 126,\; 612,\; 162,\; 216,\; 621,\; 261,\; 136,\; 613,\; 163,\; \\
316,\; 631,\; 361,\; 146,\; 614,\; 164,\; 416,\; 641,\; 461,\; 127,\; 712,\; 172,\; 217,\; 721,\; 271,\; \\
137,\; 713,\; 173,\; 317,\; 731,\; 371,\; 147,\; 714,\; 174,\; 417,\; 741,\; 471,\; 128,\; 812,\; 182,\; \\
218,\; 821,\; 281,\; 138,\; 813,\; 183,\; 318,\; 831,\; 381,\; 148,\; 814,\; 184,\; 418,\; 841,\; 481,\; \\
129,\; 912,\; 192,\; 219,\; 921,\; 291,\; 139,\; 913,\; 193,\; 319,\; 931,\; 391,\; 149,\; 914,\; 194,\; \\
419,\; 941,\; 491,\; 122,\; 212,\; 221,\; 133,\; 313,\; 331,\; 144,\; 414,\; 441,\; 112,\; 211,\; 121,\; \\
113,\; 311,\; 131,\; 114,\; 411,\; 141,\; 115,\; 511,\; 151,\; 116,\; 611,\; 161,\; 117,\; 711,\; 171,\; \\
118,\; 811,\; 181,\; 119,\; 911,\; 191,\; 111
    \end{array}
    \right\}
\end{align*}
    with $(Q_i) \in \PF^2_k$ is denoted $w_1 \cdots w_k$ with $j \in
    Q_{w_j}$ for any $j$.
\end{ex}

Let $(Q_i)$ be a $\seqPF$-parking function. We associate the \emph{underlying
composition} $\pi$ of $(Q_i)$ as the composition such that the partial sums of
cardinal of non-empty sets $Q_i$ is $\pi$.
\begin{ex}
    The underlying composition of
    $(\{2,3\},\{\},\{4\},\{\},\{\},\{1,5,6\},\{\})$ is $213$.
\end{ex}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{$\seqPF$-non-decreasing parking functions}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% With analogy with usual parking functions, a \emph{$\seqPF$-non decreasing
% parking functions} is an \emph{isomorphism type} of $\PF(\seqPF)$-structures. We
% recall the \textit{transport} of $\seqPF$-parking function $(Q_i)$ along
% bijections $\sigma$ (action of symmetric group on structures) is: $\sigma \cdot
% (Q_i) = (\sigma(Q_i))$.
% \begin{remarq}
%     In terms of functions, the transport is simply $f \circ \sigma^{-1}$.
% \end{remarq}
% The 

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Enumeration}
%%%%%%%%%%%%%%%%%%%%%%%%
From \todo{citer notre papier + thm}, the cycle index series of $\PF(\seqPF)$
is given in homogeneous $(h_\lambda)$ symmetric functions by:
\begin{align}
    Z_{\PF(\seqPF)} &= \sum_{n \seq 0} \sum_{\pi \models n} \alpha_\pi
    h_{\lambda(\pi)} 
    \qquad\text{with}\quad
    \alpha_\pi =\sum_{\tau \models \ell(\pi)}
                    \prod_{i=1}^{\ell(\tau)} \binom{\pi(\seqPF; \tau,
                    i)}{\tau_i}
    \label{eq:cycle_index_series_PF}
%\end{align*}
\intertext{where $\pi \models n$ means $\pi$ is a composition of $n$,
$\ell(\pi)$ is the number of parts of $\pi$, $\tau_i$ means the
$i^\text{th}$ part of $\tau$, $\lambda(\pi)$ is the underlying partition of
$\pi$ and}
%\begin{align*}
    \pi(\seqPF; \tau, i) &:= 
        \begin{dcases*}
        \seqPFn{1 + \sum_{j = 1}^{\tau_1 + \cdots + \tau_{i-1}} \pi_j} -
        \seqPFn{1 + \sum_{j = 1}^{\tau_1 + \cdots + \tau_{i-2}} \pi_j} & if $i
        > 1$,\\
        \seqPFn{1} & in otherwise.
        \end{dcases*}\nonumber
\end{align}
By change of basis into elementary $(e_\lambda)$-basis of symmetric functions
\todo{papier + formules}, one obtains the exponential generating series (as well
given in \cite[Theorem 4.2]{kung2003goncarov}):
\begin{align}
    \pf_\seqPF(t) = \sum_{n \seq 0} g_n\frac{t^n}{n!}\qquad\quad\text{with} \quad
    g_n = \sum_{j=1}^{n}(-1)^{j-1}\binom{n}{j}\seqPFn{n-j+1}^{j} g_{n-j}\,.
    \label{eq:sg_pf_k}
\end{align}
There is the first coefficients of $\pf$ associated to $\PF^k$ for $k = 1, 2, 3$ 
and $4$:
\begin{center}
$\begin{array}{c|l|l|l|l|l|l|l||c}
k \backslash n & 0 & 1 & 2 & 3 & 4 & 5 & 6 & \textit{OEIS} \\ 
\hline
1 & 1 & 1 & 3  & 16   & 125     & 1296        & 16807       & \oeis*{A000272} \\
2 & 1 & 1 & 7  & 142  & 5941    & 428856      & 47885899    & \oeis*{A082157} \\
3 & 1 & 1 & 15 & 1024 & 198581  & 85102056    & 68999174203 & \oeis*{A082158} \\
4 & 1 & 1 & 31 & 6766 & 5724421 & 13619068896 & 74610632873731
\end{array}$
\end{center}
\begin{remarq}
    The column for $n = 2$ is\todo{seems to be} the sequence \oeis{A183075}. 
\end{remarq}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simple $\seqPF$-parking functions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
A \emph{simple $\seqPF$-parking function} is a $\seqPF$-parking function $(Q_i)$
such that $\card{Q_i} \ieq 1$ for any $i$. We denote by $\SPF(\seqPF)$ the
(sub-)species of $\PF(\seqPF)$ with structures are simple $\seqPF$-parking
functions.
\begin{remarq}
    The simple (usual) parking functions are \textit{permutations}. 
\end{remarq} 
\begin{ex}
    The first structures $\SPF^2_n := \SPF(k^2)[n]$ for $n=1, 2$ and $3$:
\begin{align*}
    \SPF^2_1 &= \left\{
        1
    \right\}\,,\qquad
    \SPF^2_2 = \left\{
    12,\; 21,\; 13,\; 31,\; 14,\; 41
    \right\}\,,\\
    \SPF^2_3 &= \left\{\begin{array}{l}
123,\; 312,\; 132,\; 213,\; 321,\; 231,\; 124,\; 412,\; 142,\; 214,\; 421,\; 241,\; 134,\; 413,\; 143,\; \\
314,\; 431,\; 341,\; 125,\; 512,\; 152,\; 215,\; 521,\; 251,\; 135,\; 513,\; 153,\; 315,\; 531,\; 351,\; \\
145,\; 514,\; 154,\; 415,\; 541,\; 451,\; 126,\; 612,\; 162,\; 216,\; 621,\; 261,\; 136,\; 613,\; 163,\; \\
316,\; 631,\; 361,\; 146,\; 614,\; 164,\; 416,\; 641,\; 461,\; 127,\; 712,\; 172,\; 217,\; 721,\; 271,\; \\
137,\; 713,\; 173,\; 317,\; 731,\; 371,\; 147,\; 714,\; 174,\; 417,\; 741,\; 471,\; 128,\; 812,\; 182,\; \\
218,\; 821,\; 281,\; 138,\; 813,\; 183,\; 318,\; 831,\; 381,\; 148,\; 814,\; 184,\; 418,\; 841,\; 481,\; \\
129,\; 912,\; 192,\; 219,\; 921,\; 291,\; 139,\; 913,\; 193,\; 319,\; 931,\; 391,\; 149,\; 914,\; 194,\; \\
419,\; 941,\; 491
    \end{array}
    \right\}
\end{align*}
    with $(Q_i) \in \SPF^2_k$ is denoted $w_1 \cdots w_k$ with $j \in
    Q_{w_j}$ for any $j$.
\end{ex}
\begin{remarq}
    Contrary to $\PF(\seqPF)$ the species $\SPF(\seqPF)$ doesn't have
    non-trivial automorphisms.
\end{remarq}

From the constructive definition of $\seqPF$-parking functions
(\ref{eq:pf_defition_constructive}), we deduce \todo{lien papier +
interprétation} that each terms $\alpha_\pi h_{\lambda(\pi)}$ in
(\ref{eq:cycle_index_series_PF}) encodes $\seqPF$-parking functions $(Q_i)$ with
underlying composition $\pi$. That is clear that $(Q_i)$ a $\seqPF$-structure on
$[n]$ is a \emph{simple $\seqPF$-parking function} \textit{if and only if} the
underlying composition $\pi$ is $1^n$. So one obtains the cycle index serie:
\begin{align*}
    Z_{\SPF(\seqPF)} &= \sum_{n \seq 0} \sum_{\tau \models n}
    \prod_{i = 1}^{\ell(\tau)} \binom{\tau(\seqPF; i)}{\tau_i} h_{1^n}
\intertext{with}
    \tau(\seqPF; i) &= \begin{dcases*}
        \seqPFn{1 + \tau_1 + \cdots + \tau_{i-1}}
    - \seqPFn{1 + \tau_1 + \cdots + \tau_{i-2}} & if $i > 1$,\\
    \seqPFn{1} & in otherwise.
    \end{dcases*}
\end{align*}
Then it is immediate that the (exponential) generating series $\spf_\seqPF$ of
$\SPF(\seqPF)$ is:
\begin{align*}
    \spf_\seqPF(t) = \sum_{n \seq 0} \sum_{\tau \models n}
    \prod_{i = 1}^{\ell(\tau)} \binom{\tau(\seqPF; i)}{\tau_i} t^n
\end{align*}
There is the first coefficients of $\spf$ associated to $\SPF^k$ for $k = 1,2,3$
and $4$:
\begin{center}
$\begin{array}{c|l|l|l|l|l|l|l||c}
k \backslash n & 0 & 1 & 2 & 3 & 4 & 5 & 6 & \textit{OEIS} \\ 
\hline
1 & 1 & 1 & 2  & 6    & 24      & 120         & 720       & \oeis*{A000142}\\ 
2 & 1 & 1 & 6  & 108  & 4128    & 277560      & 29250720  &\\
3 & 1 & 1 & 14 & 924  & 175896  & 74526480    & 59967205200 &\\
4 & 1 & 1 & 30 & 6480 & 5459520 & 12962599200 & 70935659876160 &\\
\end{array}$
\end{center}

